A Novel Physics-based Channel Model for Reconfigurable Intelligent Surface-assisted Multi-user Communication Systems

The reconfigurable intelligent surface (RIS) is one of the promising technologies contributing to the next generation smart radio environment. A novel physics-based RIS channel model is proposed. Particularly, we consider the RIS and the scattering environment as a whole by studying the signal's multipath propagation, as well as the radiation pattern of the RIS. The model suggests that the RIS-assisted wireless channel can be approximated by a Rician distribution. Analytical expressions are derived for the shape factor and the scale factor of the distribution. For the case of continuous phase shifts, the distribution depends on the number of elements of the RIS and the observing direction of the receiver. For the case of continuous phase shifts, the distribution further depends on the quantization level of the RIS phase error. The scaling law of the average received power is obtained from the scale factor of the distribution. For the application scenarios where RIS functions as an anomalous reflector, we investigate the performance of single RIS-assisted multiple access networks for time-division multiple access (TDMA), frequency-division multiple access (FDMA) and non-orthogonal multiple access (NOMA). Closed-form expressions for the outage probability of the proposed channel model are derived. It is proved that a constant diversity order exists, which is independent of the number of RIS elements. Simulation results are presented to confirm that the proposed model applies effectively to the phased-array implemented RISs.

==> pre.tex <==
\section{Hardware Model: Phased Array-based RIS}\label{pre}

The electromagnetic characteristics of the RIS, such as phase discontinuity, can be reconfigured by tuning the surface impedance. There are various mechanisms that support this tuning. Apart from electrical voltage, other mechanisms are reported, including thermal excitation, optical pump and physical stretching. Among them, electrical control is the most convenient choice, since voltage is easier to be quantized and be controlled by FPGA chips. The choices of materials of the RIS include semiconductors~\cite{zhu2013active} and graphene~\cite{emani2015graphene}. Regardless of the different tuning mechanisms, the general geometry layout of the phased array-based RIS can be modelled as periodic unit cells integrated on a substrate. When designing RIS-assisted communication systems, the most important parameter of the RIS is the reflection coefficient $\Tilde{r}$ at each element (cell). In order to characterize tunability of the RIS, the method of equivalent lumped-element circuit can be adopted.
\begin{figure}[t!]
\centering
\includegraphics[width =3.0in]{myfig/varactor.eps}
\caption{Schemetic diagram of the varactor RIS}
\label{vara}
\end{figure}
As shown in Fig. \ref{vara}, the unit cell is equivalent to a lumped-element circuit with a load impedance of $Z_l$. Particularly, the equivalent load impedance could be tuned by changing the bias voltage of the varactor diode. According to the boundary conditions of EM fields, the reflection and transmission coefficient is determined by the impedance $Z_l$ and vacuum impedance $Z_0 \approx 377\Omega$. For the case of normal incidence, it can be shown that:
\begin{equation} \label{im}
    \Tilde{r} =\frac{\bm{E_r}}{\bm{E_i}} = \frac{Z_l-Z_0}{Z_l+Z_0},
\end{equation}
where $\Tilde{r}$ is the complex reflection coefficient, $\bm{E_r}$ and $\bm{E_i}$ are the reflected electric field and the incident electric field. \eqref{im} describes the relation between the phase discontinuity $\phi$ and equivalent surface impedance $Z_l$. As a result, discrete phase shift control can be realized by tuning $Z_l$ upon adding different levels of bias voltages. When modelling the RIS in wireless communication system designs, we can characterize each of its unit cell by the local reflection coefficients. For example, the $i$-th cell can be modelled as:
\begin{equation}\label{refl}
    \Tilde{r_i}=\beta_i \cdot e^{j\phi_i},
\end{equation}
where $\beta_i$ and $\phi_i$ correspond to amplitude control and phase control, respectively. In the following sections, $\phi(m,n)$\footnote{It is worth pointing out that the phase discontinuity denoted by $\phi$, should not be confused with other notations denoting geometrical angles, such as $\theta$,$\varphi$ or $\alpha$} refers to the phase discontinuity of the $(m,n)$-th element on the RIS, $\Tilde{r}(x,y)$ refers to the reflection coefficient as a function of the position on the RIS plane.

